Spatial Variation in Strong Line Ratios and Physical Conditions in Two Strongly-Lensed Galaxies at z~1.4

For studies of galaxy formation and evolution, one of the major benefits of the James Webb Space Telescope is that space-based IFUs like those on its NIRSpec and MIRI instruments will enable spatially resolved spectroscopy of distant galaxies, including spectroscopy at the scale of individual star-forming regions in galaxies that have been gravitationally lensed. In the meantime, there is only a very small subset of lensed sources where work like this is possible even with the Hubble Space Telescope's Wide Field Camera 3 infrared channel grisms. We examine two of these sources, SDSS J1723+3411 and SDSS J2340+2947, using HST WFC3/IR grism data and supporting spatially-unresolved spectroscopy from several ground-based instruments to explore the size of spatial variations in observed strong emission line ratios like O32, R23, which are sensitive to ionization parameter and metallicity, and the Balmer decrement as an indicator of reddening. We find significant spatial variation in the reddening and the reddening-corrected O32 and R23 values which correspond to spreads of a few tenths of a dex in ionization parameter and metallicity. We also find clear evidence of a negative radial gradient in star formation in SDSS J2340+2947 and tentative evidence of one in SDSS J1723+3411, though its star formation is quite asymmetric. Finally, we find that reddening can vary enough spatially to make spatially-resolved reddening corrections necessary in order to characterize gradients in line ratios and the physical conditions inferred from them, necessitating the use of space-based IFUs for future work on larger, more statistically robust samples.

==> ESI-stale.tex <==
We reduced the ESI two-dimensional (2D) spectra for each pointing using a combination of IRAF and Python routines. First each raw 2D frame was bias and flat-field corrected.  Cosmic rays were removed using the IRAF routine \textit{lacos}, and flux calibrations were obtained using a standard star.  Wavelength calibrations were obtained using CuAr, XeAr, and Hg arc lamps.  Apertures for the source and sky spectra were manually selected for each aperture, using the iraf apall tool; sky subtraction was done using a boxcar algorithm.  We then extracted one-dimensional order-by-order spectra from each observation of each science target, and applied the flux calibration and wavelength solution for each dispersion order.  We used custom python routines to combine all the dispersion orders to one continuous, calibrated, 1D spectrum for each science target for each night, using a noise-weighted mean in regions of order overlap.  Finally, for each object, we produced a summed 1D spectrum by combining the reduced spectra of different pointings obtained on different nights, applying the barycentric correction in the process, and weighting by the noise.

==> oldbib.tex <==
\begin{thebibliography}{}
\bibitem[Acharyya, et al.(2019)]{Acharyya:2019aa} Acharyya, A., Kewley, L. J., Rigby, J. R., et al. 2019, MNRAS, (in press) \textbf{edit this when fully published}
\bibitem[Benincasa et al.(2019)]{Benincasa2019} Benincasa, S. M., Wadsley, J. W., Couchman, H. M. P., et al. 2019, MRNAS (in press) \textbf{edit this when published, currently on arxiv} 
\bibitem[Bundy et al.(2015)]{Bundy2015} Bundy, K., Bershady, M. A., Law, D. R., et al. 2015, ApJ, 798, 7
\bibitem[Cresci et al.(2010)]{Cresci2010} Cresci, G., Mannucci, F., Maiolino, R., et al. 2010, Nature, 467, 811
\bibitem[Croom et al.(2012)]{Croom2012} Croom, S. M., Lawrence, J. S., Bland--Hawthorn, J., et al. 2012, MNRAS, 421, 872
\bibitem[Del Zanna, et al.(2015)]{DelZanna:2015aa} Del Zanna, G., Dere, K. P., Young, P. R., et al. 2015, A\&\ A, 582, 56
\bibitem[Dopita et al. (2000)]{Dopita:2000aa} Dopita, M. A., Kewley, L. J., Heisler, C. A., et al. 2000, ApJ, 542, 224
\bibitem[Dopita et al.(2013)]{Dopita:2013aa} Dopita, M. A., Sutherland, R. S., Nicholls, D. C., et al. 2013, ApJS, 208, 10
\bibitem[Elias et al.(2006)]{gnirs} Elias, J. H., Joyce, R. R., Liang, M., et al. 2006, SPIE, 6269, 138
\bibitem[Elmegreen et al.(2005)]{Elmegreens2005}Elmegreen, D. M., Elmegreen, B. G., Rubin, D.S., \& Schaffer, M.A. 2005  ApJ, 631, 85
\bibitem[F\"{o}rster-Schreiber et al.(2011)]{FoerstSch2011} F\"{o}rster-Schreiber, N.M., Shapely, A.E., Genzel, R., et al. 2011, ApJ, 739, 45
\bibitem[Genzel et al.(2008)]{Genzel2008} Genzel, R., Burkert, A., Bouch\'{e}, N., et al. 2008, ApJ, 687, 59
\bibitem[Groves et al.(2004)]{Groves:2004aa} Groves, B. A., Dopita, M. A., \& Sutherland, R. S. 2004, ApJS, 153, 9
\bibitem[Guo et al.(2012)]{Guo2012} Guo, Y., Giavalisco, M., Ferguson, H. C., et al. 2012, ApJ, 757, 120
\bibitem[Guo et al.(2018)]{GuoClumps} Guo, Y., Rafelski, M., Bell, E.F., et al. 2018, ApJ, 853, 108
\bibitem[Izotov et al.(2018)]{Izotov2018} Izotov, Y. I., Worseck, G., Schaerer, D., et al. 2018, MNRAS, 478, 4851
\bibitem[Jenkins (2009)]{Jenkins:2009aa} Jenkins, E. B. 2009, ApJ, 700, 1299
\bibitem[Johnson et al.(2017)]{Johnson2017} Johnson, T. L., Rigby, J. R., Sharon, K., et al. 2017, ApJL, 843, L21
\bibitem[Jones et al.(2010)]{Jones2010} Jones, T., Ellis, R., Jullo, E., \& Richard, J. 2010, ApJL, 725, 176
\bibitem[Kennicutt (1998)]{Kennicutt:sfr} Kennicutt, R. C., Jr. 1998, ARA\&A, 36, 189
\bibitem[Kewley \& Dopita (2002)]{KewlDop2002} Kewley, L. J., Dopita, M. A. 2002, ApJS, 142, 1, 35
\bibitem[Kewley et al.(2019a)]{Kewley:2019aa} Kewley, L. J., Nicholls, D. C., Sutherland, R. S. et al. 2019a, ApJ, (in press)
\bibitem[Kewley et al.(2019b)]{Kewley:2019ab} Kewley, L. J., Nicholls, D. C., \& Sutherland, R. S. 2019b, ARA\&\ A, (in press)
\bibitem[Levesque \& Richardson(2014)]{Levesque} Levesque, E. M. \& Richardson, M. L. A. 2014, ApJ, 780, 100
\bibitem[L\'{o}pez-S\'{a}nchez et al.(2012)]{Lopez-Sanchez:2012aa} L\'{o}pez-S\'{a}nchez, \'{A}. R., Dopita, M.C., Kewley, L. J., et al. 2012, MNRAS, 426, 2630
\bibitem[Mandelker et al.(2014)]{Mandelker2014} Mandelker, N., Dekel, A., Ceverino, D., et al. 2014, MNRAS, 443, 3675
\bibitem[Nakajima \& Ouchi (2014)]{NakaOuchi} Nakajima, K. \& Ouchi, M. 2014, MNRAS, 442, 900
\bibitem[Nakajima et al.(2013)]{NakajimaEtAl} Nakajima, K., Ouchi, M., Shimasaku, K., et al. 2013, ApJ, 769, 3
\bibitem[Nicholls et al.(2017)]{Nicholls:2017aa} Nicholls, D. C., Sutherland, R. S., Dopita, M. A., et al. 2017, MNRAS, 466, 4403
\bibitem[Onodera et al.(2016)]{Onodera} Onodera M., Carollo, C. M., Lilly, S., et al. 2016, ApJ, 822, 42
\bibitem[Patr\'{i}cio et al.(2019)]{Patricio} Patr\'{i}cio, V., Richard, J., Carton, D., et al. 2019, arXiV:1907.11586 \textbf{update when published in MNRAS}
\bibitem[Peng et al.(2002)]{Galfit} Peng, C. Y., Ho, L. C., Impey, C. D., et al. 2002, AJ, 124, 1, 266 
\bibitem[Pettini \& Pagel (2004)]{pettiniNII} Pettini, M. \& Pagel, B. E. J. 2004, MNRAS, 348, 59
\bibitem[Queyrel et al.(2012)]{Queyrel2012} Queyrel, J., Contini, T., Kissler--Patig, M. et al. 2012, A\&A, 539, A93
\bibitem[Reddy et al.(2018)]{Reddy2018} Reddy, N. A., Shapley, A. E., Sanders, R. L., et al. 2018, ApJ, 869, 92
\bibitem[Rigby et al.(2019)]{Rigby1723}  Rigby, J. R., Florian, M. K., \textbf{rest of authors}  2019, (in prep)%\apj, 588, 218
\bibitem[Rigby et al.(2011)]{Rigby0327} Rigby, J. R., Wuyts, E., Gladders, M. D., Sharon, K., \& Becker, G. D. 2011, ApJ, 732, 59
\bibitem[Rivera-Thorsen et al.(2019)]{planckArcLyC} Rivera-Thorsen, T. E., Dahle, H., Chisholm, J., et al. 2019 (submitted to Science) \textbf{update when possible}
\bibitem[Sheinis et al.(2002)]{Sheinis:2002aa} Sheinis, A. I., Bolte, M., \& Epps, H. W. 2002, PASP, 114, 851
\bibitem[Steidel et al. (2014)]{steidel2014} Steidel, C. C., Rudie, G. C., Strom, A. L., et al. 2014, ApJ, 795, 165
\bibitem[Storey \& Zeippen (2000)]{StoreyZeip} Storey, P. J., \& Zeippen, C. J., 2000, MNRAS, 312, 813
\bibitem[Stott et al.(2014)]{Stott2014} Stott, J. P., Sobral, D., Swinbank, A. M., et al. 2014, MNRAS, 443, 2695
\bibitem[Sutherland \&\ Dopita (1993)]{Sutherland:1993aa} Sutherland, R. S., \& Dopita, M. A. 1993, ApJS, 88, 253 
\bibitem[Swinbank et al.(2012)]{Swinbank2012} Swinbank, A. M., Sobral, D., Smail, I., et al. 2012, MNRAS, 426, 935
\bibitem[Tiley et al.(2019)]{Tiley2019} Tiley, A. L., Swinbank,  A. M., Harrison, C. M., et al. 2019, MNRAS, 485, 934
\bibitem[Whitaker et al.(2014)]{Whitaker0327} Whitaker, K. E., Rigby, J. R., Brammer, G. B., et al. 2014, ApJ, 790, 143 \textbf{not cited yet, but will be used when I talk about spatially-resolved SFR from Ha}
\bibitem[Wuyts et al.(2014)]{Wuyts2014} Wuyts, E., Rigby, J. R., Gladders, M. D., \& Sharon, K. 2014, ApJ, 781, 61
\end{thebibliography}
